Multivariate Intrinsic Local Polynomial Regression on Isometric Riemannian Manifolds: Applications to Positive Definite Data

The paper introduces a novel non-parametric Riemannian regression method using Isometric Riemannian Manifolds (IRMs). The proposed technique, Intrinsic Local Polynomial Regression on IRMs (ILPR-IRMs), enables global data mapping between Riemannian manifolds while preserving underlying geometries. The ILPR method is generalized to handle multivariate covariates on any Riemannian manifold and isometry. Specifically, for manifolds equipped with Euclidean Pullback Metrics (EPMs), a closed analytical formula is derived for the multivariate ILPR (ILPR-EPM). Asymptotic statistical properties of the ILPR-EPM for the multivariate local linear case are established, including a formula for the asymptotic bias, establishing estimator consistency. The paper showcases possible applications of the method by focusing on a group of Riemannian metrics on the Symmetric Positive Definite (SPD) manifold, which arises in machine learning and neuroscience. It is demonstrated that several metrics on the SPD manifold are EPMs, resulting in a closed analytical expression for the multivariate ILPR estimator on the SPD manifold. The paper evaluates the ILPR estimator's performance under two specific EPMs, Log-Cholesky and Log-Euclidean, on simulated data on the SPD manifold and compares it with extrinsic LPR using the Affine-Invariant when scaling the manifold and covariate dimension. The results show that the ILPR using the Log-Cholesky metric is computationally faster and provides a better trade-off between error and time than other metrics. Finally, the Log-Cholesky metric on the SPD manifold is employed to implement an efficient and intrinsic version of Rie-SNE for visualizing high-dimensional SPD data. The code for implementing ILPR-EPMs and other relevant calculations is available on the GitHub page.

==> CUP-JNL-DTM.tex <==
%%
%% This is file `CUP-JNL-DTM.cls',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% classes.dtx  (with options: `CUP-JNL-DTM')
%%
%% This is a generated file.
%%
%% Copyright 1993 1994 1995 1996 1997 1998 1999 2000 2001 2002 2003 2004 2005 2006 2007 2008 2009
%% The LaTeX3 Project and any individual authors listed elsewhere
%% in this file.
%%
%% This file was generated from file(s) of the LaTeX base system.
%% --------------------------------------------------------------
%%
%% It may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3c
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%    http://www.latex-project.org/lppl.txt
%% and version 1.3c or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This file has the LPPL maintenance status "maintained".
%%
%% This file may only be distributed together with a copy of the LaTeX
%% base system. You may however distribute the LaTeX base system without
%% such generated files.
%%
%% The list of all files belonging to the LaTeX base distribution is
%% given in the file `manifest.txt'. See also `legal.txt' for additional
%% information.
%%
%% The list of derived (unpacked) files belonging to the distribution
%% and covered by LPPL is defined by the unpacking scripts (with
%% extension .ins) which are part of the distribution.
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
\NeedsTeXFormat{LaTeX2e}[1995/12/01]
\ProvidesClass{CUP-JNL-DTM}
[2020/05/04 v0.1: An authoring template for CUP DTM articles]

\newif\if@restonecol
\newif\if@titlepage   \@titlepagefalse
\newif\if@cropmarkson \@cropmarksonfalse

%% Template Options
\DeclareOption{a4paper}{\PassOptionsToPackage{a4}{crop}}
\DeclareOption{a3paper}{\PassOptionsToClass{a3paper}{article}\PassOptionsToPackage{a3}{crop}}
\DeclareOption{centre}{\PassOptionsToPackage{center}{crop}}
\DeclareOption{crop}{\PassOptionsToPackage{frame}{crop}\global\@cropmarksontrue}
\DeclareOption{nocrop}{\PassOptionsToPackage{off}{crop}\global\@cropmarksontrue}
\DeclareOption{info}{\PassOptionsToPackage{info}{crop}}
\DeclareOption{noinfo}{\PassOptionsToPackage{noinfo}{crop}}

%% Classfile Options
\DeclareOption{oneside}{\@twosidefalse \@mparswitchfalse}
\DeclareOption{twoside}{\@twosidetrue  \@mparswitchtrue}
\DeclareOption{draft}{\setlength\overfullrule{5pt}}
\DeclareOption{titlepage}{\@titlepagetrue}
\DeclareOption{notitlepage}{\@titlepagefalse}
\DeclareOption{onecolumn}{\@twocolumnfalse}
\DeclareOption{twocolumn}{\@twocolumntrue}
\DeclareOption{openbib}{\let\if@openbib\iftrue}

\ExecuteOptions{twosidecrop,crop,centre,info,croppage}
\ProcessOptions
\LoadClass[twoside,fleqn]{article}

%% General Packages Used
\RequirePackage{url}
\RequirePackage{soul}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%% Fonts & Sizes %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
\DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}
\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}
\DeclareOldFontCommand{\sl}{\normalfont\slshape}{\@nomath\sl}
\DeclareOldFontCommand{\sc}{\normalfont\scshape}{\@nomath\sc}
\DeclareRobustCommand*\cal{\@fontswitch\relax\mathcal}
\DeclareRobustCommand*\mit{\@fontswitch\relax\mathnormal}

\renewcommand\normalsize{%
	\@setfontsize\normalsize{10pt}{12pt}%
	\abovedisplayskip 9.5\p@ \@plus2\p@ \@minus0\p@
	\abovedisplayshortskip 3\p@ \@plus3\p@%
	\belowdisplayshortskip 9.5\p@ \@plus3\p@ \@minus3\p@%
	\belowdisplayskip \abovedisplayskip%
	\let\@listi\@listI}%
\normalsize
\newcommand\medsize{%
	\@setfontsize\small\@xipt{13}%
	\abovedisplayskip 5\p@ \@plus3\p@ \@minus4\p@
	\abovedisplayshortskip \z@ \@plus2\p@
	\belowdisplayshortskip 3\p@ \@plus2\p@ \@minus2\p@
	\def\@listi{\leftmargin\leftmargini
		\topsep 4\p@ \@plus2\p@ \@minus2\p@
		\parsep 2\p@ \@plus\p@ \@minus\p@
		\itemsep \parsep}%
	\belowdisplayskip \abovedisplayskip}
\renewcommand\small{%
	\@setfontsize\small\@ixpt{11}%
	\abovedisplayskip 5\p@ \@plus3\p@ \@minus4\p@
	\abovedisplayshortskip \z@ \@plus2\p@
	\belowdisplayshortskip 3\p@ \@plus2\p@ \@minus2\p@
	\def\@listi{\leftmargin\leftmargini
		\topsep 4\p@ \@plus2\p@ \@minus2\p@
		\parsep 2\p@ \@plus\p@ \@minus\p@
		\itemsep \parsep}%
	\belowdisplayskip \abovedisplayskip}
\renewcommand\footnotesize{%
	\@setfontsize\footnotesize{7}{8}%
	\abovedisplayskip 5\p@ \@plus2\p@ \@minus4\p@
	\abovedisplayshortskip \z@ \@plus\p@
	\belowdisplayshortskip 3\p@ \@plus\p@ \@minus2\p@
	\def\@listi{\leftmargin\leftmargini
		\topsep 3\p@ \@plus\p@ \@minus\p@
		\parsep 2\p@ \@plus\p@ \@minus\p@
		\itemsep \parsep}%
	\belowdisplayskip \abovedisplayskip}
%
\renewcommand\scriptsize{\@setfontsize\scriptsize\@ixpt\@ixpt}
\newcommand\scrisize{\@setfontsize\scrisize{9.3}{9}}
\renewcommand\tiny{\@setfontsize\tiny\@vpt\@vipt}
\renewcommand\large{\@setfontsize\large{12}{14}}
\newcommand\larg{\@setfontsize\larg{11}{13}}
\renewcommand\Large{\@setfontsize\Large{16}{18}}
\renewcommand\LARGE{\@setfontsize\LARGE\@xviipt{22}}
\renewcommand\huge{\@setfontsize\huge\@xxpt{25}}
\renewcommand\Huge{\@setfontsize\Huge\@xxvpt{30}}
%
\DeclareMathSizes{\@ixpt}{\@ixpt}{7}{5}
\DeclareMathSizes{\@xpt}{\@xpt}{7}{5}
\DeclareMathSizes{\@xipt}{\@xipt}{7}{5}

\DeclareRobustCommand*\textsubscript[1]{%
	\@textsubscript{\selectfont#1}}%
\def\@textsubscript#1{%
	{\m@th\ensuremath{_{\mbox{\fontsize\sf@size\z@#1}}}}}

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%% Layout Settings %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

\RequirePackage{geometry}

%% Regular Pages (for Opening page - redefined)
\geometry{%
	paperwidth=174mm,
	paperheight=247mm,
	top={57pt},
	headheight={7pt},
	headsep={19.5pt},
	textwidth={144mm},
	textheight={612.5pt},
	marginparsep=3mm,
	marginparwidth=10mm,
	bindingoffset=6mm,
	footskip=0mm}
%

\setlength{\marginparsep}{3mm}%
\setlength{\marginparwidth}{10mm}%

\setlength\footskip{0\p@}
\setlength\maxdepth{0pt}

\setlength\footnotesep{5.75\p@}
\setlength{\skip\footins}{8\p@ \@plus 4\p@ \@minus 0\p@}

\setlength\parindent{12pt}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%% Pagination Settings %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Line spacing
\setlength\lineskip{1\p@}
\setlength\normallineskip{1\p@}
\renewcommand\baselinestretch{}
\parskip=0pt

% Page break penalties
\@lowpenalty   51
\@medpenalty  151
\@highpenalty 301

% Disallow widows and orphans
\clubpenalty 10000
\widowpenalty 10000

% Disable page breaks before equations, allow pagebreaks after
% equations and discourage widow lines before equations.
\displaywidowpenalty 100
\predisplaypenalty   10000
\postdisplaypenalty  0

% Set these global demerits
\doublehyphendemerits 1000000   % corresponds to badness 800
\finalhyphendemerits  1000000  % corresponds to badness 1000

% Allow loose lines rather than overfull lines
\vbadness=9999
\tolerance=9999

% Allow breaking the page in the middle of a paragraph
\interlinepenalty 0

% Disallow breaking the page after a hyphenated line
\brokenpenalty 10000

% Hyphenation; don't split words into less than three characters
\lefthyphenmin=3
\righthyphenmin=3

% Float placement parameters

% The total number of floats that can be allowed on a page.
\setcounter{totalnumber}{10}

% The maximum number of floats at the top and bottom of a page.
\setcounter{topnumber}{5}
\setcounter{bottomnumber}{5}

% The maximum part of the top or bottom of a text page that can be
% occupied by floats. This is set so that at least four lines of text
% fit on the page.
\renewcommand\topfraction{.921}
\renewcommand\bottomfraction{.921}

% The minimum amount of a text page that must be occupied by text.
% This should accomodate four lines of text.
\renewcommand\textfraction{.13}

% The minimum amount of a float page that must be occupied by floats.
\renewcommand\floatpagefraction{.887}

% The same parameters repeated for double column output
\renewcommand\dbltopfraction{.88}
\renewcommand\dblfloatpagefraction{.88}

% Space between floats
\setlength\floatsep    {18\p@ \@plus 2\p@ \@minus 2\p@}

% Space between floats and text
\setlength\textfloatsep{19\p@ \@plus 2\p@ \@minus 4\p@}

% Space above and below an inline figure
\setlength\intextsep   {18\p@ \@plus 2\p@ \@minus 2\p@}

% For double column floats
\setlength\dblfloatsep    {20\p@ \@plus 2\p@ \@minus 2\p@}
\setlength\dbltextfloatsep{18\p@ \@plus 2\p@ \@minus 4\p@}

\hyphenation{Figure Figures Table Tables Equation Equations Section Sections Appendix Theorem Lemma}

%
%%%%%%%%%%%%%%%%%%%%%%%%%%% Math Settings %%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%% For above/below spacing  
\def\eqnarray{%
	\stepcounter{equation}%
	\def\@currentlabel{\p@equation\theequation}%
	\global\@eqnswtrue
	\m@th
	\global\@eqcnt\z@
	\tabskip\@centering
	\let\\\@eqncr
	$$\everycr{}\halign to\displaywidth\bgroup
	\hskip\@centering$\displaystyle\tabskip\z@skip{##}$\@eqnsel
	&\global\@eqcnt\@ne\hskip \tw@\arraycolsep \hfil${##}$\hfil
	&\global\@eqcnt\tw@ \hskip \tw@\arraycolsep
	$\displaystyle{##}$\hfil\tabskip\@centering
	&\global\@eqcnt\thr@@ \hb@xt@\z@\bgroup\hss##\egroup
	\tabskip\z@skip
	\cr
}
\def\endeqnarray{%
	\@@eqncr
	\egroup
	\global\advance\c@equation\m@ne
	$$\@ignoretrue
}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%% Titles %%%%%%%%%%%%%%%%%%%%%%%%%%%
%

\renewcommand\contentsname{Contents}
\renewcommand\listfigurename{List of Figures}
\renewcommand\listtablename{List of Tables}
\renewcommand\refname{References}
\renewcommand\indexname{Index}
\renewcommand\figurename{Figure}
\renewcommand\tablename{Table}
\renewcommand\partname{Part}
\renewcommand\appendixname{Appendix}
\renewcommand\abstractname{Abstract}

%
%%%%%%%%%%%%%%%%%%%%%%%%%%% Article Front Matter %%%%%%%%%%%%%%%%%%%%%%%%%%%
%

%% Article Type
\sodef\letterspacetwty{}{.1em}{.4em plus1em}{.5em plus 1em minus1em }
\def\articletype#1{\gdef\ArtType{\letterspacetwty{#1}}\gdef\@ArtType{#1}}%
\articletype{RESEARCH ARTICLE}%

%% Meta Info
%\def\@artid{xx}
%\def\@jname{xxx xxx}
%\def\@jvol{xx}
%\def\@jissue{xx}
%\def\@jyear{{0000}}
%\def\@jmonth{xx}
%\def\@DOI{}
%\def\@logourl{}
%
\def\artid#1{\gdef\@artid{#1}}
\def\jname#1{\markboth{\textit{#1}}{\textit{#1}}\gdef\@jname{#1}}
\def\jvol#1{\gdef\@jvol{#1}}
\def\jissue#1{\gdef\@jissue{#1}}
\def\jyear#1{\gdef\@jyear{#1}}
\def\jmonth#1{\gdef\@jmonth{#1}}
\def\jdoi#1{\gdef\@DOI{doi:#1}\gdef\@logourl{#1}}
% \jdoi{10.4153/xxxx}
\jname{Data/Math}%
%

%%% Font Def
\def\Titlefont{\fontfamily{\rmdefault}\fontsize{16}{18}\fontseries{b}\selectfont}
\def\Artcatfont{\fontfamily{\rmdefault}\fontsize{8.5}{10.5}\fontseries{b}\selectfont}
\def\Authorfont{\fontsize{10}{12}\selectfont}
\def\addressfont{\fontsize{8}{10}\selectfont\raggedright}
\def\abstractheadfont{\fontfamily{\rmdefault}\fontsize{9}{11}\fontseries{b}\selectfont}%
\def\abstractsubheadfont{\fontfamily{\rmdefault}\fontsize{9}{11}\fontseries{b}\selectfont}%
\def\abstractfont{\fontsize{9}{11}\selectfont}%
\def\keywordfont{\fontsize{8}{10}\selectfont}%
\def\historyfont{\fontsize{8}{10}\selectfont\raggedright}

%% Article Title
%\def\title#1{\gdef\@title{#1}}

\renewcommand{\title}[2][]{%
	\gdef\@checktitle{#1}\ifx\@checktitle\empty\gdef\@title{#2}
	\gdef\s@title{#2}\else\gdef\@title{#2}\gdef\s@title{#1}\fi}

%% Cross Link for Author & Address
\def\jmkLabel#1{\@bsphack\protected@write\@auxout{}{\string\Newlabel{#1}{\@currentlabel}}\@esphack}
\def\Newlabel#1#2{\expandafter\xdef\csname X@#1\endcsname{#2}}
\def\jmkRef#1{\@ifundefined{X@#1}{0}{\csname X@#1\endcsname}}

%% Article Author(s)
\let\sep\@empty%
\let\authorsep\@empty%
\newcount\aucount%
\newcount\punctcount%
\def\author{\advance\aucount by 1\@ifstar\@@corrauthor\@@author}%
\def\au@and{\ifnum\punctcount=2\ and\else\unskip,\advance\punctcount by -1 \fi}%
\def\artauthors{}
\newif\if@auemail%
\newcommand{\@@author}[2][]{\g@addto@macro\artauthors{%
		\ifnum\aucount=1%
		\global\@auemailtrue%
		\else%
		\global\@auemailfalse%
		\fi%
		\Authorfont%
		\def\baselinestretch{1}%
		\authorsep{#2}\unskip\ifx#1\empty\else\textsuperscript{\smash{{%
					\@for\@@affmark:=#1\do{\edef\affnum{\@ifundefined{X@\@@affmark}{1}{\jmkRef{\@@affmark}}}%
						\unskip\sep\affnum\let\sep=,}}}}\fi%
		\def\authorsep{\au@and~}%%% 
		\global\let\sep\@empty\global\let\@corref\@empty%
	}}%
	
	\newcommand{\@@corrauthor}[2][]{\g@addto@macro\artauthors{%
			\global\@auemailtrue%
			\Authorfont%
			\def\baselinestretch{1}%
			\authorsep{#2}\unskip\ifx#1\empty\else\textsuperscript{\smash{{%
						\@for\@@affmark:=#1\do{\edef\affnum{\@ifundefined{X@\@@affmark}{1}{\jmkRef{\@@affmark}}}%
							\unskip\sep\affnum\let\sep=,}}}}\fi%
			\def\authorsep{\au@and~}%%% 
			\global\let\sep\@empty\global\let\@corref\@empty%
		}}%
		%
		\RequirePackage{ltxcmds}%
		\def\authororcid#1{%
			\ltx@ifpackageloaded{hyperref}{\href{https://orcid.org/#1}{\includegraphics{orcid_logo}}}{{\includegraphics{orcid_logo}}}%
		}
		\newcommand{\orcid}[1]{\protect\g@addto@macro\artauthors{%
				\authororcid{#1}%
			}}
			%
			%% Author Email
			\newif\ifcorrauth
			\def\addressrule{\kern-10\p@ \hrule \@height.15pt \@width\marginparwidth \kern 1.6\p@}%
			\def\@email{}
			\DeclareUrlCommand\myemail{}%
			\def\email#1{ {\hbox{E-mail:}~}\ltx@ifpackageloaded{hyperref}{\textcolor{blue}}{}{\protect\myemail{#1}}}%
			\let\nomail\relax
			
			%% Corrseponding Address 
			\def\@copycorthanks{}
			\def\auaddress{}
			\def\@auaddress{}
			\newcounter{affn}
			\renewcommand\theaffn{\arabic{affn}}
			\def\address{\@ifstar\@@coraddress\@@address}
			\newcount\addcount% To check the count of address
			\newcommand{\@@coraddress}[2][]{%\advance\addcount by 1
				\g@addto@macro\auaddress{%
					\stepcounter{affn}%
					\xdef\@currentlabel{\theaffn}%
					\jmkLabel{\theaffn}%
					{\textsuperscript{#1}#2.}\par}
			}
			
			%% Author Address 
			\def\addsep{\par\vskip0pt}
			\newcount\addcount% To check the count of address
			\newcommand{\@@address}[2][]{\advance\addcount by 1\g@addto@macro\auaddress{%
					\stepcounter{affn}%
					\xdef\@currentlabel{\theaffn}%
					\jmkLabel{\theaffn}%
					{\textsuperscript{#1}#2.}\par}%\theaffn
			}
			
			
			%% Address tagging 
			\newcommand{\orgdiv}[1]{#1}%
			\newcommand{\orgname}[1]{#1}%
			\newcommand{\orgaddress}[1]{#1}%
			\newcommand{\street}[1]{#1}
			\newcommand{\postcode}[1]{#1}
			\newcommand{\city}[1]{#1}
			\newcommand{\state}[1]{#1}
			\newcommand{\country}[1]{#1}
			
			%% Author name in Running Head
			\def\@authormark{}% 
			\def\authormark#1{\markright{{{#1}}}\gdef\@authormark{\def\etal{{et al.}}#1}\gdef\@authormarkforcite{\def\etal{\textit{et al.}}#1}}%
			\def\etal{\textit{et al.}}
			
			%% Optional Text
			\def\artnotefont{\reset@font\fontfamily{\rmdefault}\fontsize{8.6}{13}\selectfont\raggedright}
			\def\artnote#1{\gdef\@Artnote{#1}}\artnote{}%
			
			%% Article Abstract
			\newcommand\abstracthead{\@startsection {section}{1}{\z@}{-22pt \@plus2ex \@minus0ex}{0.0001pt}{\abstractheadfont}}
			\newcommand\subabstracthead{\@startsection{subsection}{2}{\z@}{3pt \@plus0ex \@minus0ex}{-.5em}{\abstractsubheadfont}}
			
			\def\@abstract{}%
			\long\def\abstract#1{\def\@abstract{%
					\let\paragraph\subabstracthead%
					\abstractfont%
					\abstracthead*{\abstractname}%
					#1\par}}%
			
			\def\printabstract{\ifx\@abstract\empty\else\@abstract\fi\par}%
			
			\def\printkeywords{\ifx\@keywords\empty\else\@keywords\fi\par}%
			
			%
			%% Keywords
			\def\keywordname{Keywords}
			\newcommand{\keywords}[2][\keywordname]{%
				\g@addto@macro\@keywords{\par\addvspace{5pt}{\keywordfont\textbf{#1:} #2\par}}}
			\def\@keywords{}
			\newcommand{\codes}[2][Primary]{\textit{#1} -- #2}%
			
			%% Article History
			
			\newcommand{\received}[2][Received:]{\g@addto@macro\@history{{\textbf{#1} #2}}}%
			\newcommand{\revised}[2][Revised:]{\g@addto@macro\@history{{; \textbf{#1} #2}}}%
			\newcommand{\accepted}[2][Accepted:]{\g@addto@macro\@history{{; \textbf{#1} #2}}}%
			
			%% Article Header Definition
			\renewcommand{\@maketitle}
			{\noindent{\vbox{%
						\hsize\textwidth\parindent0pt%
						\vskip7pt%
						%% Aritle Type
						{\hbox to \textwidth{{\Artcatfont\ArtType\hfill}\par}}
						% {\vskip5pt\hbox to \textwidth{\ltx@ifpackageloaded{hyperref}{\href{https://crossmark.crossref.org/dialog?doi=\@logourl}}{}{\includegraphics{CrossRef-logo}}\par}}
						%% Aritle Title
						\ifx\@title\empty\else%
						\vskip15.5pt%
						{\Titlefont\@title\par}
						%\addcontentsline{toc}{chapter}{\@title}% for bookmarks
						\fi%
						%% Aritle Authors, Address and Correspondings
						\ifnum\aucount>0
						\global\punctcount\aucount%
						\vskip10pt%
						\artauthors\par%%     authors and emails
						{\vskip7pt\addressfont\auaddress\par%%      corresponding adress
							%\corremail\par
						}
						\fi%
						% {\printhistory\par}%
						{\printkeywords\par}%
						{\printabstract\par}%
					}}\par\addvspace{23pt plus0pt minus0pt}}
				
				%% Printing Article Header
				\renewcommand\maketitle{\par
					\@afterindentfalse%
					\begingroup
					\gdef\UrlFont{\rmfamily}%
					\renewcommand\thefootnote{\@fnsymbol\c@footnote}%
					\def\@makefnmark{\rlap{\@textsuperscript{\normalfont\smash{\@thefnmark}}}}%
					\long\def\@makefntext##1{\parindent 1em\noindent\small\selectfont
						\hbox{\@textsuperscript{\normalfont\@thefnmark}}##1}%
					\if@twocolumn
					\ifnum \col@number=\@ne%
					\twocolumn[\@maketitle]%
					\else
					\twocolumn[\@maketitle]%
					\fi%
					\else%
					\newpage%
					\global\@topnum\z@% Prevents figures from going at top of page.
					\@maketitle%
					\fi%
					\thispagestyle{titlepage}%
					\endgroup%
					\global\advance\opshortpage23pt%
					\enlargethispage{-38pt}%  
					\setcounter{footnote}{0}%
					\global\let\thanks\relax%
					\global\let\maketitle\relax%
					\global\let\@maketitle\relax%
					%\global\let\@thanks\@empty%
					\global\let\@author\@empty%
					\global\let\@date\@empty%
					%\global\let\@title\@empty%
					\global\let\title\relax%
					\global\let\author\relax%
					\global\let\date\relax%
					\global\let\and\relax
					%%%print continuous abstract on next page
					\@afterheading}%
				
				
				\newenvironment{Frontmatter}{\par}{\maketitle\par}
				
				\newenvironment{Backmatter}{\par\fontsize{8}{10}\selectfont
					\def\sectionfont{\fontfamily{\rmdefault}\fontsize{10}{12}\fontseries{b}\selectfont\raggedright}
					\def\paragraphfont{\fontfamily{\rmdefault}\fontsize{8}{10}\fontseries{b}\selectfont\raggedright\boldmath}
					\renewcommand\section{\@startsection {section}{1}{\z@}%
						{-12pt \@plus -2ex \@minus 0ex}%
						{3pt}%
						{\sectionfont}}%
					\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
						{2.25ex \@plus1ex \@minus.2ex}%
						{-.5em}%
						{\paragraphfont}}
					\def\bibfont{\fontsize{8}{10}\selectfont}%
				}{\par}
				\def\bysame{\leavevmode\hbox to3em{\hrulefill}}
				
				%
				%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Page Styles %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
				%
				\def\opheaderfont{\fontsize{7}{9}\selectfont}
				\def\headerfont{\fontsize{10}{12}\selectfont}
				\def\footerfont{\fontsize{7}{8}\selectfont}
				
				
				%% Regular Page Style      
				\def\ps@headings{%
					\def\@oddfoot{\hfill}
					\let\@evenfoot\@oddfoot
					\def\@evenhead{{\headerfont \thepage\qquad\textit{\rightmark}\hfill}}%
					\def\@oddhead{{\headerfont \hfill\textit{\leftmark}\qquad\thepage}}%
					\let\@mkboth\markboth%
				}
				
				\newdimen\opshortpage%
				
				\def\printcopyright#1{#1}%%
				
				\def\copytext#1{\def\@copyrighttext{\begin{minipage}[t]{\textwidth}\footerfont #1\end{minipage}}}
				\copytext{\textcopyright\ The Author(s) 2020. This is an Open Access article, distributed under the terms of the Creative Commons Attribution licence (http://
					creativecommons.org/licenses/by/4.0/), which permits unrestricted re-use, distribution, and reproduction in any medium, provided the original work is
					properly cited.
				}%
				
				\AtEndDocument{\label{LastPage}}
				\def\@opjournalheader{\textit{\@jname}\space\ {{(\@jyear),\ \textbf{\@jvol}:\@artid}} {\thepage{--}\pageref*{LastPage}}\\
					{\@DOI}}%
				
				%% Opening Page Style      
				\def\ps@titlepage{%
					\def\@oddhead{{\hbox to \textwidth{%
								\vbox to 0pt{\vskip-5pt\rlap{\hbox to \textwidth{\hfill\includegraphics[scale=.75]{CUP_Logo}
											%   \quad\includegraphics{DataMath_Logo}
											\hspace*{-1pt}}}}%
								\vbox to 0pt{\vskip-7pt\rlap{\parbox{\textwidth}{\opheaderfont\begin{tabular*}{\textwidth}[b]{@{\extracolsep{\fill}}@{}l@{}}%
												\@opjournalheader%
											\end{tabular*}}}}%
										}}}%
										\let\@evenhead\@oddhead%
										%  \def\@oddfoot{\vbox to 0pt{\vskip-\opshortpage{\printcopyright{\@copyrighttext}}}}%%
										\let\@evenfoot\@oddfoot}%
									
									%
									%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Sections %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
									%
									\def\numbered{\setcounter{secnumdepth}{3}}
									\def\unnumbered{\setcounter{secnumdepth}{0}}
									\numbered%% default is unnumbered Sections
									
									\newcounter {chapter}[part]% for bookmarks
									\renewcommand\thepart         {\@Roman\c@part}
									\renewcommand\thesection      {\@arabic\c@section}
									\renewcommand\thesubsection   {\thesection.\@arabic\c@subsection}
									\renewcommand\thesubsubsection{\thesubsection.\@arabic\c@subsubsection}
									\renewcommand\theparagraph    {\thesubsubsection.\@arabic\c@paragraph}
									\renewcommand\thesubparagraph {\theparagraph.\@arabic\c@subparagraph}
									%%
									\renewcommand\part{\par
										\addvspace{4ex}%
										\@afterindentfalse
										\secdef\@part\@spart}
									%%
									\def\@part[#1]#2{%
										\ifnum \c@secnumdepth >\m@ne
										\refstepcounter{part}%
										\addcontentsline{toc}{part}{\thepart\hspace{1em}#1}%
										\else
										\addcontentsline{toc}{part}{#1}%
										\fi
										{\parindent \z@ \raggedright
											\interlinepenalty \@M
											\normalfont
											\ifnum \c@secnumdepth >\m@ne
											\Large\bfseries \partname~\thepart
											\par\nobreak
											\fi
											\huge \bfseries #2%
											\markboth{}{}\par}%
										\nobreak
										\vskip 3ex
										\@afterheading}
									
									\def\@spart#1{%
										{\parindent \z@ \raggedright
											\interlinepenalty \@M
											\normalfont
											\huge \bfseries #1\par}%
										\nobreak
										\vskip 3ex
										\@afterheading}
									
									\def\@sect#1#2#3#4#5#6[#7]#8{%
										\ifnum #2>\c@secnumdepth
										\let\@svsec\@empty
										\else
										\refstepcounter{#1}%
										\protected@edef\@svsec{\@seccntformat{#1}\relax}%
										\fi
										\@tempskipa #5\relax
										\ifdim \@tempskipa>\z@
										\begingroup
										#6{%
											\@hangfrom{\hskip #3\relax\@svsec}%
											\interlinepenalty \@M #8\@@par}%
										\endgroup
										\csname #1mark\endcsname{#7}%
										\addcontentsline{toc}{#1}{%
											\ifnum #2>\c@secnumdepth \else
											\protect\numberline{\csname the#1\endcsname}%
											\fi
											#7}%
										\else
										\def\@svsechd{%
											#6{\hskip #3\relax
												\@svsec #8.}%
											\csname #1mark\endcsname{#7}%
											\addcontentsline{toc}{#1}{%
												\ifnum #2>\c@secnumdepth \else
												\protect\numberline{\csname the#1\endcsname}%
												\fi
												#7}}%
										\fi
										\@xsect{#5}}
									%
									\def\sectionfont{\fontfamily{\rmdefault}\fontsize{10}{12}\fontseries{b}\selectfont\raggedright}
									\def\subsectionfont{\fontfamily{\rmdefault}\fontsize{10}{12}\fontseries{b}\fontshape{it}\selectfont\raggedright}
									\def\subsubsectionfont{\fontfamily{\rmdefault}\fontsize{9.5}{11.5}\fontseries{b}\selectfont\raggedright}
									\def\paragraphfont{\fontfamily{\rmdefault}\fontsize{9.5}{11.5}\fontshape{it}\selectfont\raggedright\boldmath}
									\def\subparagraphfont{\fontfamily{\rmdefault}\fontsize{10}{12}\fontseries{b}\fontshape{it}\selectfont\raggedright}
									
									\def\@seccntformat#1{{\csname the#1\endcsname.}\hskip.5em}
									
									\renewcommand\section{\@startsection {section}{1}{\z@}%
										{-18pt \@plus -2ex \@minus 0ex}%
										{6pt}%
										{\sectionfont}}
									\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
										{-18pt \@plus 0ex \@minus 0ex}%
										{6pt}%
										{\subsectionfont}}
									\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
										{-12.5pt \@plus 0ex \@minus 0ex}%
										{0.001pt}%
										{\subsubsectionfont}}
									\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
										{12.5pt \@plus1ex \@minus.2ex}%
										{0.0001pt}%
										{\paragraphfont}}
									\renewcommand\subparagraph{\@startsection{subparagraph}{5}{\z@}%
										{-6pt \@plus1ex \@minus .2ex}%
										{-1em}%
										{\subparagraphfont}}
									%
									\def\@startsection#1#2#3#4#5#6{%
										\if@noskipsec \leavevmode \fi
										\par
										\@tempskipa #4\relax
										\@afterindenttrue
										\ifdim \@tempskipa <\z@
										\@tempskipa -\@tempskipa \@afterindentfalse
										\fi
										\if@nobreak
										\everypar{}\ifnum#2=2\vskip0pt\else\ifnum#2=3\vskip1pt\else\ifnum#2=4\vskip1pt\fi\fi\fi%
										\else
										\addpenalty\@secpenalty\addvspace\@tempskipa
										\fi
										\@ifstar
										{\@ssect{#3}{#4}{#5}{#6}}%
										{\@dblarg{\@sect{#1}{#2}{#3}{#4}{#5}{#6}}}}
									%
									%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Lists %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
									%
									
									\newdimen\labelwidthi
									\newdimen\labelwidthii
									\newdimen\labelwidthiii
									\newdimen\labelwidthiv
									\def\normal@labelsep{0.5em}
									\labelsep\normal@labelsep
									\settowidth{\labelwidthi}{(iii)}
									\settowidth{\labelwidthii}{(d)}
									\settowidth{\labelwidthiii}{(iii)}
									\settowidth{\labelwidthiv}{(M)}
									\leftmargini\labelwidthi    \advance\leftmargini\labelsep
									\leftmarginii\labelwidthii  \advance\leftmarginii\labelsep
									\leftmarginiii\labelwidthiii \advance\leftmarginiii\labelsep
									\leftmarginiv\labelwidthiv  \advance\leftmarginiv\labelsep
									\def\setleftmargin#1#2{\settowidth{\@tempdima}{#2}\labelsep\normal@labelsep
										\csname labelwidth#1\endcsname\@tempdima
										\@tempdimb\@tempdima \advance\@tempdimb\labelsep
										\csname leftmargin#1\endcsname\@tempdimb}
									\def\@listI{\leftmargin\leftmargini
										\labelwidth\labelwidthi \labelsep\normal@labelsep
										\topsep 6pt \partopsep\z@ \parsep\z@ \itemsep\z@
										\listparindent 1em}
									\def\@listii{\leftmargin\leftmarginii
										\labelwidth\labelwidthii \labelsep\normal@labelsep
										\topsep\z@ \partopsep\z@ \parsep\z@ \itemsep\z@
										\listparindent 1em}
									\def\@listiii{\leftmargin\leftmarginiii
										\labelwidth\labelwidthiii \labelsep\normal@labelsep
										\topsep\z@ \partopsep\z@ \parsep\z@ \itemsep\z@
										\listparindent 1em}
									\def\@listiv{\leftmargin\leftmarginiv
										\labelwidth\labelwidthiv \labelsep\normal@labelsep
										\topsep\z@ \partopsep\z@ \parsep\z@ \itemsep\z@
										\listparindent 1em}
									\let\@listi\@listI
									\@listi
									%
									\setlength  \labelsep  {.5em}
									\setlength  \labelwidth{\leftmargini}
									\addtolength\labelwidth{-\labelsep}
									\@beginparpenalty -\@lowpenalty
									\@endparpenalty   -\@lowpenalty
									\@itempenalty     -\@lowpenalty
									\def\labelitemi{$\bullet$}          \def\labelitemii{$\cdot$}
									\def\labelenumi{\theenumi.}        \def\theenumi{\arabic{enumi}}
									\def\labelenumii{(\alph{enumii})}   \def\theenumii{\theenumi\alph{enumii}}
									\def\labelenumiii{(\roman{enumiii})}\def\theenumiii{\theenumii.\roman{enumiii}}
									\def\labelenumiv{(\Alph{enumiv})}   \def\theenumiv{\theenumiii.\Alph{enumiv}}
									
									%
									%%%%%%%%%%%%%%%%%%%%%%%%%%% Ordered & Unordered List  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
									%
									
									\def\listfont{\selectfont}%
									
									\def\enumargs{%
										\listfont%
										\leftmargini0pt%
										\topsep 6pt%
										\partopsep     \z@%
										\itemsep       \z@%
										\parsep        \z@%
										\labelsep      .5em%
										\rightmargin   \z@%
										\raggedright%   
										\listparindent \parindent%
										\itemindent    \z@}%
									
									\def\enumerate{%
										\@ifnextchar[{\@numerate}{\@numerate[0.]}}
									
									\def\@numerate[#1]{\par%
										\ifnum \@enumdepth >3 \@toodeep\else
										\advance\@enumdepth \@ne
										\edef\@enumctr{enum\romannumeral\the\@enumdepth}
										\list{\csname label\@enumctr\endcsname}{%
											\enumargs%
											\setlength{\leftmargin}{\csname leftmargin\romannumeral\the\@enumdepth\endcsname}
											\usecounter{\@enumctr}
											\settowidth\labelwidth{#1}
											\addtolength{\leftmargin}{\labelwidth}
											\addtolength{\leftmargin}{\labelsep}
											\def\makelabel##1{\hss\llap{##1}}}%
										\fi
									}
									\let\endenumerate\endlist
									
									%%Unnumbered list%%
									\def\unenumargs{%
										\listfont%
										\leftmargini\parindent%
										\topsep6pt%
										\partopsep     \z@%
										\itemsep       \z@%
										\parsep        \z@%
										\labelsep      0\p@%
										\rightmargin   \z@%
										\raggedright%
										\listparindent \parindent%
										\itemindent    -10pt}%
									
									\def\unenumerate{%
										\@ifnextchar[{\@unenumerate}{\@unenumerate[0.]}}
									
									\def\@unenumerate[#1]{\par%
										\ifnum \@enumdepth >3 \@toodeep\else
										\advance\@enumdepth \@ne
										\edef\@enumctr{enum\romannumeral\the\@enumdepth}
										\list{\csname label\@enumctr\endcsname}{%
											\unenumargs
											\setlength{\leftmargin}{\csname leftmargin\romannumeral\the\@enumdepth\endcsname}
											\usecounter{\@enumctr}
											\settowidth\labelwidth{#1}
											\addtolength{\leftmargin}{\labelwidth}
											\addtolength{\leftmargin}{\labelsep}
											\def\makelabel##1{\hss\llap{##1}}}%
										\fi
									}
									\let\endunenumerate\endlist%
									
									\def\itemargs{%
										\listfont%
										\leftmargini-1.5pt%
										\topsep6pt%
										\partopsep     \z@%
										\itemsep       \z@%
										\parsep        \z@%
										\labelsep      .5em%
										\rightmargin   \z@%
										\raggedright%
										\listparindent \parindent%
										\itemindent    \z@}%
									
									\renewcommand\labelitemi{\textbullet}
									\renewcommand\labelitemii{\textendash}
									
									\def\itemize{%
										\@ifnextchar[{\@itemize}{\@itemize[$\bullet$]}}
									
									\def\@itemize[#1]{\par%
										\ifnum \@itemdepth >3 \@toodeep\else
										\advance\@itemdepth \@ne
										\edef\@itemctr{item\romannumeral\the\@itemdepth}
										\list{\csname label\@itemctr\endcsname}{%
											\itemargs
											\setlength{\leftmargin}{\csname leftmargin\romannumeral\the\@itemdepth\endcsname}
											\settowidth\labelwidth{#1}
											\addtolength{\leftmargin}{\labelwidth}
											\addtolength{\leftmargin}{\labelsep}
											\def\makelabel##1{\hss \llap{##1}}}%
										\fi
									}
									\let\enditemize\endlist
									%
									\def\verse{\let\\=\@centercr
										\list{}{\itemsep\z@
											\itemindent \z@
											\listparindent\z@
											\rightmargin 1em
											\leftmargin \rightmargin}\item[]}
									\let\endverse\endlist
									\def\quotation{\list{}{\vskip 8pt\itemindent\z@
											\leftmargin 1em \rightmargin \z@
											\parsep \z@ \@plus 1pt}\item[]}
									\newcommand\e{\endlist\vskip 8pt}
									\let\endquotation\e
									\def\quote{\list{}{\itemindent\z@
											\leftmargin 1em \rightmargin \z@}%
										\item[]}
									\let\endquote\endlist
									\def\descriptionlabel#1{\hspace\labelsep\bfseries #1}
									\def\description{\list{}{\leftmargin=2em\labelwidth\z@
											\leftmargin \z@ \topsep6pt\itemindent-\leftmargin
											%\advance\itemindent-\labelsep
											\let\makelabel\descriptionlabel}}
									\let\enddescription\endlist
									%
									%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Float %%%%%%%%%%%%%%%%%%%%%%%%%%%%
									
									\setlength\abovecaptionskip{2.25\p@}
									\setlength\belowcaptionskip{3\p@}
									
									\setlength\arraycolsep{2\p@}
									\setlength\tabcolsep{6\p@}
									\setlength\arrayrulewidth{.4\p@}
									\setlength\doublerulesep{2\p@}
									\setlength\tabbingsep{\labelsep}
									
									\def\fnum@figure{{\figurename}\space\relax{\thefigure}}
									\def\fnum@table{{\tablename}\space\relax{\thetable}}
									
									\def\FigName{figure}
									
									\long\def\@makecaption#1#2{%
										\ifx\FigName\@captype
										\vskip\abovecaptionskip
										\@figurecaption{#1}{#2}
										\else
										\@tablecaption{#1}{#2}
										\vskip\belowcaptionskip
										\fi%
									}
									
									
									%% Figure
									
									\def\figurenumfont{\reset@font\fontfamily{\rmdefault}\fontsize{10}{12}\fontshape{it}\fontseries{b}\selectfont}
									\def\figurecaptionfont{\fontfamily{\rmdefault}\fontsize{10}{12}\fontshape{it}\selectfont}
									
									\newdimen\figwidth%
									\newdimen\figheight%
									\newdimen\sidecapwidth
									\newdimen\wrapcapline%
									\newdimen\totalwrapline%
									\newdimen\wraptotline%
									
									%% Figures macro
									\def\FIG#1#2{%
										{\centering#1\par}
										#2}
									
									%% Figures caption
									\newbox\figcapbox
									\newbox\capbox
									\long\def\@figurecaption#1#2{%
										{%
											\setbox\figcapbox\hbox{\figurecaptionfont{\figurenumfont #1}\hskip.5em#2.\vphantom{y}\par}
											%% Caption printing depending on figure width
											\ifdim\wd\figcapbox>\textwidth
											{\figurecaptionfont{\figurenumfont #1.}\hskip.5em{#2}.\par}%
											\else%
											{\figurecaptionfont\centering{\figurenumfont #1.}\hskip.5em{#2}.\par}%
											\fi%
										}}%
										
										%
										%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
										%
										\RequirePackage{booktabs}
										\cmidrulewidth=.15pt%
										%
										\def\tablenumfont{\reset@font\fontsize{10}{12}\fontshape{it}\fontseries{b}\selectfont}
										\def\tablecaptionfont{\fontsize{10}{12}\fontshape{it}\selectfont}
										\def\tablebodyfont{\fontsize{10}{12}\selectfont}
										\def\tablecolheadfont{\fontsize{10}{12}\selectfont}
										\def\tablefootnotefont{\fontsize{7}{8}\selectfont\raggedright}
										
										%% Table Macro
										\newbox\tablebox
										%\newdimen\tabbodywidth
										\long\def\TBL#1#2{%
											\renewcommand\arraystretch{1}%
											%\setbox\tablebox\hbox{\tablebodyfont #2\par}
											%\tabbodywidth\wd\tablebox%
											#1\vskip 0pt%
											{\tablebodyfont #2\par}%
										}
										
										%% Table Caption
										\newbox\tabcapbox
										\newdimen\tabcapwidth
										\long\def\@tablecaption#1#2{%
											{\setbox\tabcapbox\hbox{\tablecaptionfont{\tablenumfont #1.}\hskip.5em#2.\vphantom{y}\endgraf}%
												\tabcapwidth\wd\tabcapbox%
												\ifdim\tabcapwidth<\hsize%
												{\tablecaptionfont\centering{\tablenumfont #1.}\hskip.5em#2.\vphantom{y}\par}%
												\else
												{\tablecaptionfont{\tablenumfont #1.}\hskip.5em#2.\vphantom{y}\par}%
												\fi}}%
										
										%% Table Column Heads
										\def\TCH#1{{\tablecolheadfont #1}}
										
										%% Table Footnotes
										\newenvironment{fntable}[1][\columnwidth]{%
											\def\@makefnmark{\hbox{\@textsuperscript{\fontsize{5}{5}\selectfont\@thefnmark}}}%
											\begin{minipage}{#1}%
												\def\thempfootnote{{\@arabic\c@mpfootnote}}
												%%%%%%%%%%
												\def\@xfootnotemark[##1]{%
													\begingroup
													%\c@footnote #1\relax
													\unrestored@protected@xdef\@thefnmark{##1}%
													\endgroup
													\@footnotemark}
												%%%%%%%%%
												\def\@xfootnotenext[##1]{%
													\begingroup
													%\csname c@\@mpfn\endcsname ##1\relax
													\unrestored@protected@xdef\@thefnmark{##1}%
													\endgroup
													\@footnotetext}
												\renewcommand\@makefntext[1]{{%
														\tablefootnotefont%
														\hskip0pt{\smash{\@makefnmark}}##1\par}}
												\renewcommand\footnotesize{\@setfontsize\footnotesize{7}{8.5}}%
											}%
											{\vspace{-0.75\skip\footins}%
												\renewcommand{\footnoterule}{}%
											\end{minipage}}%
											
											%% Table Rules
											\def\toprule{%\noalign{\vskip3pt}
												\noalign{\ifnum0=`}\fi
												\hrule \@height 0\p@ \@width 0pt
												\hrule \@height .15\p@ % <- rule height
												\hrule \@height 5pt \@width 0pt
												\futurelet\@tempa\@xhline}
											% Middle rule
											\def\midrule{\noalign{\ifnum0=`}\fi%
												\hrule \@height 3pt \@width 0pt
												\hrule \@height .15pt % <- rule height
												\hrule \@height 5pt \@width 0pt
												\futurelet \@tempa\@xhline}
											% Bottom rule
											\def\botrule{\noalign{\ifnum0=`}\fi
												\hrule \@height 3pt \@width 0pt
												\hrule \@height .15\p@ % <- rule height
												\futurelet\@tempa\@xhline}
											%
											\def\@@@cmidrule[#1-#2]#3#4{\global\@cmidla#1\relax
												\global\advance\@cmidla\m@ne
												\ifnum\@cmidla>0\global\let\@gtempa\@cmidrulea\else
												\global\let\@gtempa\@cmidruleb\fi
												\global\@cmidlb#2\relax
												\global\advance\@cmidlb-\@cmidla
												\global\@thisrulewidth=#3
												\@setrulekerning{#4}
												\ifnum\@lastruleclass=\z@\vskip 3\p@\fi
												\ifnum0=`{\fi}\@gtempa
												\noalign{\ifnum0=`}\fi\futurenonspacelet\@tempa\@xcmidrule}
											\def\@xcmidrule{%
												\ifx\@tempa\cmidrule
												\vskip-\@thisrulewidth
												\global\@lastruleclass=\@ne
												\else \ifx\@tempa\morecmidrules
												\vskip \cmidrulesep
												\global\@lastruleclass=\@ne\else
												\vskip 5\p@
												\global\@lastruleclass=\z@
												\fi\fi
												\ifnum0=`{\fi}}
											\let\cline\cmidrule
											
											%
											%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
											%
											
											\renewcommand\@pnumwidth{1.55em}
											\renewcommand\@tocrmarg{2.55em}
											\renewcommand\@dotsep{4.5}
											\setcounter{tocdepth}{3}
											\renewcommand\tableofcontents{%
												\section*{\contentsname
													\@mkboth{%
														\MakeUppercase\contentsname}{\MakeUppercase\contentsname}}%
												\@starttoc{toc}%
											}
											\renewcommand*\l@part[2]{%
												\ifnum \c@tocdepth >-2\relax
												\addpenalty\@secpenalty
												\addvspace{2.25em \@plus\p@}%
												\begingroup
												\setlength\@tempdima{3em}%
												\parindent \z@ \rightskip \@pnumwidth
												\parfillskip -\@pnumwidth
												{\leavevmode
													\large \bfseries #1\hfil \hb@xt@\@pnumwidth{\hss #2}}\par
												\nobreak
												\if@compatibility
												\global\@nobreaktrue
												\everypar{\global\@nobreakfalse\everypar{}}%
												\fi
												\endgroup
												\fi}
											\renewcommand*\l@section[2]{%
												\ifnum \c@tocdepth >\z@
												\addpenalty\@secpenalty
												\addvspace{0em}% \@plus\p@}%
												\setlength\@tempdima{1.5em}%
												\begingroup
												\parindent \z@ \rightskip \@pnumwidth
												\parfillskip -\@pnumwidth
												\leavevmode \bfseries
												\advance\leftskip\@tempdima
												\hskip -\leftskip
												#1\nobreak\hfil \nobreak\hb@xt@\@pnumwidth{\hss #2}\par
												\endgroup
												\fi}
											\renewcommand*\l@subsection{\@dottedtocline{2}{1.5em}{2.3em}}
											\renewcommand*\l@subsubsection{\@dottedtocline{3}{3.8em}{3.2em}}
											\renewcommand*\l@paragraph{\@dottedtocline{4}{7.0em}{4.1em}}
											\renewcommand*\l@subparagraph{\@dottedtocline{5}{10em}{5em}}
											\renewcommand\listoffigures{%
												\section*{\listfigurename
													\@mkboth{\MakeUppercase\listfigurename}%
													{\MakeUppercase\listfigurename}}%
												\@starttoc{lof}%
											}
											\renewcommand*\l@figure{\@dottedtocline{1}{1.5em}{2.3em}}
											\renewcommand\listoftables{%
												\section*{\listtablename
													\@mkboth{%
														\MakeUppercase\listtablename}{\MakeUppercase\listtablename}}%
												\@starttoc{lot}%
											}
											\let\l@table\l@figure
											
											%
											%%%%%%%%%%%%%%%%%%%%%%%%%%%% Mini-TOC %%%%%%%%%%%%%%%%%%%%%%%%%
											%
											\RequirePackage{etoc}
											\etocarticlestylenomarks
											%
											%%%%%%%%%%%%%%%%%%%%%%%%%%%% Other Env. %%%%%%%%%%%%%%%%%%%%%%%%%
											%
											
											\renewenvironment{quote}
											{\list{}{\topsep=0pt\topsep6pt\leftmargin=1em\raggedright}%
												\item\relax}
											{\endlist}
											
											
											%
											%%%%%%%%%%%%%%%%%%%%%%%%%%%% Appendix %%%%%%%%%%%%%%%%%%%%%%%%%
											%
											
											\newif\ifbackmatter%
											\newcommand{\backmatter}{\par\global\backmattertrue}
											
											%
											%%%%%%%%%%%%%%%%%%%%%%%%%%%% Appendix %%%%%%%%%%%%%%%%%%%%%%%%%
											%
											%
											%%%%%%%%%%%%%%%%%%%%%%%%%%%% BackMatters %%%%%%%%%%%%%%%%%%%%%%%%%
											%
											%
											%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
											%
											
											
											%
											%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Doi-Links %%%%%%%%%%%%%%%%%%%%%%%%%%%
											%
											%% From doi.sty %%
											
											\DeclareRobustCommand{\doitext}{{doi}:}%
											
											%% the meat of the code
											%% the first command opens a group, and changes a few catcodes.
											\newcommand*{\DOI}{%
												\begingroup
												\lccode`\~=`\#\relax
												\lowercase{\def~{\#}}%
												\lccode`\~=`\_\relax
												\lowercase{\def~{\_}}%
												\lccode`\~=`\<\relax
												\lowercase{\def~{\textless}}%
												\lccode`\~=`\>\relax
												\lowercase{\def~{\textgreater}}%
												\lccode`\~=0\relax
												\catcode`\#=\active
												\catcode`\_=\active
												\catcode`\<=\active
												\catcode`\>=\active
												\doitext\@mydoi
											}
											
											%% this is the actual command which processes the argument, with the catcodes
											%% set in the previous command
											%% it closes the group, and spits out the url.
											\def\@mydoi#1{%
												\let\#\relax
												\let\_\relax
												\let\textless\relax
												\let\textgreater\relax
												\edef\x{\toks0={{#1}}}%
												\x
												\edef\#{\@percentchar23}%
												\edef\_{_}%
												\edef\textless{\@percentchar3C}% instead of {\string<} for Apple
												\edef\textgreater{\@percentchar3E}% instead of {\sting>} for Apple
												\edef\x{\toks1={\noexpand\href{http://dx.doi.org/#1}}}%
												\x
												\edef\x{\endgroup\the\toks1 \the\toks0}%
												\x
											}
											%
											%%%%%%%%%%%%%%%%%%%%%%%%%%% Article History  %%%%%%%%%%%%%%%%%%%%
											%
											\def\@history{}
											\def\printhistory{{\par\addvspace{5pt}%
													\historyfont\noindent%
													\ifx\@history\empty\gdef\@history{Received xx xxx xxxx}\fi\@history\par}
											}%
											
											%
											\renewenvironment{theindex}
											{\if@twocolumn
												\@restonecolfalse
												\else
												\@restonecoltrue
												\fi
												\columnseprule \z@
												\columnsep 35\p@
												\twocolumn[\section*{\indexname}]%
												\@mkboth{\MakeUppercase\indexname}%
												{\MakeUppercase\indexname}%
												\thispagestyle{plain}\parindent\z@
												\parskip\z@ \@plus .3\p@\relax
												\let\item\@idxitem}
											{\if@restonecol\onecolumn\else\clearpage\fi}
											\renewcommand\@idxitem{\par\hangindent 40\p@}
											\renewcommand\subitem{\@idxitem \hspace*{20\p@}}
											\renewcommand\subsubitem{\@idxitem \hspace*{30\p@}}
											\renewcommand\indexspace{\par \vskip 10\p@ \@plus5\p@ \@minus3\p@\relax}
											
											%
											%%%%%%%%%%%%%%%%%%%%%%% Footnotes %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
											%
											
											\renewcommand\footnoterule{%
												\kern2\p@%
												\hrule \@height.15pt \@width5pc%
												\kern4.5\p@}%
											%
											
											\def\@makefnmark{{\textsuperscript{\@thefnmark}}}
											
											\renewcommand\@makefntext[1]{%
												\hskip8pt{\smash{\@makefnmark}}#1}
											%
											\AtBeginDocument{%
												\@ifpackageloaded{hyperref}{%
													\RequirePackage{hypcap}%
													\renewcommand\UrlFont{\rmfamily}%
												}{}%
												%
												\@ifpackageloaded{natbib}{%
													\renewcommand\bibsection{%
														\section*{\refname}%
														\vspace*{3pt}%
													}%
												}{}%
											}%
											
											\def\doi#1{\quad\url{http://dx.doi.org/#1}}
											%
											%
											%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
											%
											
											\pagestyle{headings}
											\pagenumbering{arabic}
											\sloppy
											\frenchspacing
											\flushbottom
											
											%%% special parameters for TeX
											\linepenalty=100
											
											\endinput
											

